SCOTT: Self-Consistent Chain-of-Thought Distillation

Large language models (LMs) beyond a certain scale, demonstrate the emergent capability of generating free-text rationales for their predictions via chain-of-thought (CoT) prompting. While CoT can yield dramatically improved performance, such gains are only observed for sufficiently large LMs. Even more concerning, there is little guarantee that the generated rationales are consistent with LM's predictions or faithfully justify the decisions. In this work, we propose a faithful knowledge distillation method to learn a small, self-consistent CoT model from a teacher model that is orders of magnitude larger. To form better supervision, we elicit rationales supporting the gold answers from a large LM (teacher) by contrastive decoding, which encourages the teacher to generate tokens that become more plausible only when the answer is considered. To ensure faithful distillation, we use the teacher-generated rationales to learn a student LM with a counterfactual reasoning objective, which prevents the student from ignoring the rationales to make inconsistent predictions. Experiments show that, while yielding comparable end-task performance, our method can generate CoT rationales that are more faithful than baselines do. Further analysis suggests that such a model respects the rationales more when making decisions; thus, we can improve its performance more by refining its rationales.

==> tables/error_pattern_gpt3.tex <==
\begin{table}[t]
%\vspace{-0.7cm}
\centering
% \vspace{0.3cm}
\scalebox{0.85}{
\begin{tabular}{l}
\toprule[1.5pt]
\textbf{Error 1} ($42\%$): Do not provide new information. \\
\midrule
\textbf{Q}: Can a Bengal cat survive eating only pancakes? \\
\textbf{A}: The answer is no. This is because: \textit{\textcolor{blue}{A Bengal}} \\
\textit{\textcolor{blue}{~~~~~cat cannot survive eating only pancakes.}}\\
\midrule[1.5pt]
\textbf{Error 2}  ($37\%$): Do not justify the answer.\\
\midrule
\textbf{Q}: Is material from an aloe plant sometimes \\
~~~~~enclosed in petroleum-derived products? \\
\textbf{A}: The answer is yes.
This is because: \textit{\textcolor{blue}{Aloe is a plant.}}\\ 
\textit{\textcolor{blue}{~~~~~Plants are made of cells. Cells are made of molecules.}} \\
\textit{\textcolor{blue}{~~~~~Molecules are made of atoms.}} \\
\bottomrule[1.5pt]
\end{tabular}
}
\caption{\textbf{Vacuous rationales} (\textcolor{blue}{blue}) generated by a prompted LM (GPT-3) for StrategyQA. Out of 100 random rationales, we found: (1) $42\%$ of them do not provide new information not contained in the task input. (2) $37\%$ of them do not justify the answer.
\xiang{I’m also wishing to transform Table 1 to a more compelling figure, where you could still quote the two numbers about the two kinds of dominant errors. Sth using icons and putting CoT into color-coded ways like below would look better?}
}
\label{tab:error_gpt3}
\end{table}
